Lepton Flavour Symmetries

We provide a general classification of flavour symmetries according to their interplay with the proper Poincare' and gauge groups and to their linear or nonlinear action in field space. We focus on the lepton sector and we review the different types of symmetries describing neutrino masses and the lepton mixing matrix. For each type of symmetry we present several illustrative examples and we discuss specific strengths and limitations.

==> CPoriginal.tex <==
The main purpose of including CP transformations in the flavour symmetry group is to constrain Majorana phases. There are several dedicated reviews on this topic, such as for example \cite{King:2014nza,Neder:2015wsa,King:2015aea,Hagedorn:2017icd,King:2017guk,Petcov:2017ggy,Coloma:2018ioo}. 
In a theory invariant under both a flavour symmetry group $G_f$ and CP, besides eq.~(\ref{eq:mLinvariancePhi}), the following constraint holds for the lepton mass matrices:\footnote{In the presence of a single Higgs, a possible phase in its CP transformation can be reabsorbed in the transformation of the lepton fields.}
\begin{eqnarray}
M^*_E(\phi) &=& X_{e^c}^T\, M_E(X_\phi\phi^*) \, X_l \nn\\
m^*_\nu(\phi) &=&X_l^T\, m_\nu(X_\phi\phi^*) X_l \;,
\label{eq:mLinvarianceCP}
\end{eqnarray}
where we have denoted with $X_f$ $(f=e^c,l,\phi)$ unitary matrices describing the action of CP on the field $f$ and we have assumed Majorana neutrinos.
In such a theory CP can only be broken spontaneously and the conditions that realize the breaking are
\begin{itemize}
 \item[{\em  i})] $X_\phi\phi^*\ne \phi$ on the vacuum.
 \item[{\em ii})] No other consistent CP transformation leaving 
invariant both the theory and the vacuum exists.
\end{itemize}
\subsection{Sequestering and residual symmetries}
As in the case of a flavour symmetry commuting with the proper Poincar\'e group, to some extent it is possible to analyze the predictions of the theory without referring to an
explicit realization, relying on the residual symmetries enjoyed by the charged lepton sector and by the neutrino sector, if any. Provided $M_E$ and $m_\nu$ depend 
on two separate sets of flavons, $\phi_E$ and $\phi_\nu$, we can contemplate independent residual symmetries for the two sectors:
\be
U_\phi(g_E)\phi_E=\phi_E \hspace{2cm} U_\phi(g_\nu)\phi_\nu=\phi_\nu \;,
\ee 
where $g_E$ and $g_\nu$ run in different subgroups of $G_f$ and these relations hold in the vacuum. To constrain Majorana phases we should further assume that CP is conserved in the neutrino sector:
\be
X_\phi\phi^*_\nu=\phi_\nu \;.
\ee 
By combining eqs.~(\ref{eq:mLinvariancePhi}) and~(\ref{eq:mLinvarianceCP}), we end up with the relations:
\be
(M_E^\dagger M_E)=\rep_l(g_E)^\dagger (M_E^\dagger M_E) \rep_l(g_E) \; , \qquad m_\nu = \rep_l(g_\nu)^T m_\nu \, \rep_l(g_\nu) \;, \qquad m^*_\nu =X_l^T\, m_\nu X_l \;,
\ee
which constrain at the same time the lepton mixing angles and both Dirac and Majorana phases. 
\begin{table}[h!] 
\centering
\begin{tabular}{|c|c|c|}
\hline
$G_e$&$G_\nu$&\#{\tt parameters}\rule[-2ex]{0pt}{5ex}\\
\hline
$Z_{m_1}\times \ldots \times Z_{m_p}$&$Z_2\times Z_2\times \text{CP}$&0\rule[-2ex]{0pt}{5ex}\\
\hline
$Z_{m_1}\times \ldots \times Z_{m_p}$&$Z_2\times \text{CP}$&1\rule[-2ex]{0pt}{5ex}\\
\hline
$Z_2\times \text{CP}$&$Z_2\times Z_2\times \text{CP}$&1\rule[-2ex]{0pt}{5ex}\\
\hline
$Z_2\times \text{CP}'$&$Z_2\times \text{CP}$&2\rule[-2ex]{0pt}{5ex}\\
\hline
$Z_{m_1}\times \ldots \times Z_{m_p}$&$\text{CP}$&3\rule[-2ex]{0pt}{5ex}\\
\hline
$Z_2$&$Z_2\times \text{CP}$&3\rule[-2ex]{0pt}{5ex}\\
\hline
\end{tabular}
\caption{Number of continuous free parameters describing the lepton mixing matrix $U(\theta_{ij},\delta,\alpha_{21},\alpha_{31})$ \cite{Chen:2014wxa,Lu:2016jit}. In the first and second column, the residual symmetries $G_e$ and $G_\nu$
of the charged lepton sector and the neutrino sector, respectively. The cyclic symmetry $Z_{m_1}\times \ldots \times Z_{m_p}$ is assumed to fully distinguish the charged leptons
by their different transformation properties.
The residual symmetry $Z_2\times Z_2\times \text{CP}$ is also equivalent to the one generated by the four allowed CP transformations of the neutrino sector, see the text. In the fourth line, CP and $\text{CP}'$ are in general independent CP transformations.}
\label{tableCP}
\end{table}

This program has been carried out in the context of discrete flavour symmetry groups
$G_f$. A variety of cases arises from the different possible assignments of the residual symmetries.
Assuming three generations, in the neutrino sector the most general group leaving neutrino masses unconstrained is the Klein group $Z_2\times Z_2$.
To avoid mass degeneracies \footnote{Degeneracies in the neutrino mass spectrum in this context have been anayzed in ref.~\cite{Joshipura:2018cpb}.}, the matrix $X_l$ is required to be symmetric: $X_l^T = X_l$ \cite{Feruglio:2012cw}. Since $X_l$ is also unitary, this automatically implies $\text{CP}^2=1$ \footnote{In Section \ref{roleCP} we have seen that $(X^*_l X^{\phantom{*}}_l)^n = 1$ holds for a finite group.}. To guarantee that the action of CP on lepton electroweak doublets is always represented by a symmetric matrix, $X_l$ is required to commute with the four elements of the Klein group. Given the antilinear action of CP, commutation is
expressed through relations of the type: 
\be
X_l \, U(g_K)^*=U(g_K) \, X_l \;,
\label{XZ}
\ee
where $g_K$ stands for an element of the Klein group. Indeed $X'_l=U(g_K) \, X_l$ represents just another CP transformation and eq.~(\ref{XZ}) implies that the matrix $X'_l$
is symmetric.
It also follows that four CP transformations can be selected as residual symmetries of the neutrino sector.
Conversely, given these four allowed CP transformations, the Klein group can be fully reconstructed \cite{Chen:2014wxa,Everett:2016jsk}.
Usually the group $G_e$ consists of a direct product of cyclic symmetries, $Z_{m_1}\times \ldots \times Z_{m_p}$, such that all the charged leptons
are distinguished by their different 
transformation properties. Among the residual symmetries of the charged lepton sector there can also be an accidental CP symmetry, independent from the one acting in the neutrino sector.

\subsection{Parameter counting}

The freedom in the definition of the model gives rise to many cases and, depending on the specific set of assumptions, the PMNS matrix is determined up to a number of continuous free parameters, listed in table \ref{tableCP}. 
These parameters arise as follows. The invariance under CP provides, in a suitable basis,
a reality condition on the neutrino mass matrix, which can be parametrized in terms of three masses and three angles. An additional $Z_2\times Z_2$ symmetry fully determines these angles, while a single parity $Z_2$ leaves one angle unconstrained. The three angles remain free parameters if the only residual symmetry of the neutrino sector is CP.
In the charged lepton sector the choice $G_e=Z_{m_1}\times \ldots \times Z_{m_p}$, when all leptons have different transformation properties, leaves no free parameters beyond masses. One free angle originates from $G_e=Z_2\times \text{CP}$ and one angle and one phase from $G_e=Z_2$. Adding the parameters of the two sectors reproduces table \ref{tableCP}. 
This approach leaves lepton masses unconstrained, and
the PMNS matrix is always determined up to permutations of rows and columns.
Moreover the intrinsic parity of neutrinos, that is the relative sign of their masses, cannot
be established. As a result the physical phases are fixed modulo $\pi$.
\subsection{Examples}
\subsubsection{$\mu-\tau$ reflection symmetry}
A simple example is provided by the so called $\mu-\tau$ reflection symmetry
\cite{Harrison:2002kp,Harrison:2002et,Grimus:2003yn,Harrison:2004he}\footnote{See \cite{Zhou:2014sya,Mohapatra:2015gwa,Joshipura:2015dsa,Zhao:2017yvw,Rodejohann:2017lre,Nishi:2018vlz,Sinha:2018xof} for more recent applications related to the topic of this section.}. In the basis where the charged lepton mass matrix is diagonal and ordered
from smaller to bigger masses, the CP transformation
acting on neutrinos is specified by:
\be
X_l=
\left(
\begin{array}{ccc}
1&0&0\\
0&0&1\\
0&1&0
\end{array}
\right) \;,
\ee
and the constraint $m^*_\nu =X_l^T\, m_\nu X_l$ implies the relations $\sin\theta_{23}=1/\sqrt{2}$, $\sin\theta_{12}\cos\theta_{12}\sin\theta_{13}\cos\delta=0$ and $\sin\alpha_{21}=\sin\alpha_{31}=0$. Data requires $\sin\theta_{12}\cos\theta_{12}\sin\theta_{13}\ne 0$ and this scheme predicts a maximal Dirac CP phase, $|\sin\delta|=1$.
\subsubsection{$G=S_4\rtimes \text{CP}$}
If we assume  $G_e=Z_{m_1}\times \ldots \times Z_{m_p}$ and 
 $G_\nu=Z_2\times \text{CP}$
in the neutrino sector, see the second row of table \ref{tableCP}, the PMNS matrix depends on a continuous parameter.  An example is provided by $G=S_4\rtimes \text{CP}$, $G_e=Z_3$  \cite{Feruglio:2012cw}. Due to the different embedding of the $Z_2$ subgroup in $S_4$, there are five inequivalent choices of $Z_2\times \text{CP}$ transformations leaving the neutrino sector invariant. Four of them, labelled I, II, IV and V, reproduce particular cases of the so-called trimaximal mixing pattern.

Models I and II reproduce $U_{\text{TM}_2}$, while  Models IV and V give rise to $U_{\text{TM}_1}$, with $\phi$, $\alpha,\beta$ (see \Sect{loose}) quantized and assuming only the values shown in table \ref{tableCP1}.
Models I  and IV predict maximal atmospheric mixing angle, maximal Dirac CP violation, trivial CP Majorana phases and provide two realizations of the $\mu-\tau$ 
reflection symmetry enjoying an additional prediction.
Model II and V predict no lepton CP violation of Dirac or Majorana type. The relations (\ref{eq:relTM2}) 
apply to model I(II) with $|\cos\delta|=0(1)$.
\begin{table}[h!] 
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
{\tt Model}& {\tt Pattern}& $|\sin\phi|$ & $\sin\alpha$ & $\sin\beta$&$\sin^2\theta_{23}$&$\sin^2\theta_{13}$&$\sin^2\theta_{12}$&$|\sin\delta|$&$\sin\alpha_{21}$&$\sin\alpha_{31}$\rule[-3ex]{0pt}{7ex}\\
\hline
I& $\text{TM}_2$& $1$ & $0$ & $0$&$\dd\frac{1}{2}$&$\dd\frac{2}{3}\sin^2\theta$&$\dd\frac{1}{2+\cos 2\theta}$&$1$&$0$&$0$\rule[-3ex]{0pt}{7ex}\\
\hline
II& $\text{TM}_2$&$0$ & $0$ & $0$&$\dd\frac{1}{2}\left(1\pm\frac{\sqrt{3}\sin 2\theta}{2+\cos 2\theta}\right)$&$\dd\frac{2}{3}\sin^2\theta$&$\dd\frac{1}{2+\cos 2\theta}$&$0$&$0$&$0$\rule[-3ex]{0pt}{7ex}\\
\hline
IV& $\text{TM}_1$&$1$ & $0$ & $0$&$\dd\frac{1}{2}$&$\dd\frac{\sin^2\theta}{3}$&$\dd\frac{\cos^2\theta}{2+\cos^2\theta}$&$1$&$0$&$0$ \rule[-3ex]{0pt}{7ex}\\
\hline
V& $\text{TM}_1$&$0$ & $0$ & $0$&$\dd\frac{1}{2}(1\mp\frac{2\sqrt{6}\sin 2\theta}{5+\cos 2\theta})$&$\dd\frac{\sin^2\theta}{3}$&$\dd\frac{\cos^2\theta}{2+\cos^2\theta}$&$0$&$0$&$0$ \rule[-3ex]{0pt}{7ex}\\
\hline
\end{tabular}
\caption{Specific mixing pattern arising in four out of the five independent cases arising from $S_4$ and CP invariance, broken down to $Z_3$ in the charged lepton sector and to $Z_2\times \text{CP}$ in the neutrino sector $G=S_4\rtimes \text{CP}$  \cite{Feruglio:2012cw} as a function of the parameters $\theta\in [0,\pi/2]$.}
\label{tableCP1}
\end{table}
A general property of $\text{TM}_2$ is $\sin^2\theta_{12}>1/3$.
By letting $\sin^2\theta_{13}$ vary in its 3$\sigma$ allowed range, the first relation predicts $\sin^2\theta_{12}=0.340\div0.342$, presently allowed within 3$\sigma$,
but out of the 2$\sigma$ range. 
In model II, $\tan^2\delta=0$ and the 3$\sigma$ allowed range of $\sin^2\theta_{13}$ results in $\sin^2\theta_{23}=\{0.388\div0.398\} \cup \{0.602\div0.611\}$. The prediction falling in the first octant is excluded at 3$\sigma$, whereas the one falling in the second octant is allowed at 2$\sigma$. A vanishing $\sin\delta$ is disfavored by the current data, but it is not excluded at 3$\sigma$. The relations (\ref{eq:relTM1}) for model IV(V) require $|\cos\delta|=0(1)$.
In $\text{TM}_1$ we always have $\sin^2\theta_{12}<1/3$.
By letting $\sin^2\theta_{13}$ vary in its 3$\sigma$ allowed range, the first relation predicts $\sin^2\theta_{12}=0.316\div0.319$, in very good agreement with present data. Model V is ruled out since the second relation with $\tan^2\delta=0$ leads to values of $\sin^2\theta_{23}$ excluded by data. The quoted ranges have been derived from the results of the global fit in \cite{Esteban:2018azc}. The group $G=A_4\rtimes \text{CP}$ leads to the $\text{TM}_2$ mixing pattern shown in table \ref{tableCP2}, with $|\sin\phi|=0$ or $|\sin\phi|=1$ and $\sin\alpha=\sin\beta=0$ as for models I and II \cite{Feruglio:2012cw,Ding:2013bpa,Nishi:2016jqg,Li:2016nap}.
Explicit models have been constructed for this case in ref.~\cite{Ding:2013bpa,Li:2016nap}.
Starting from $G=S_4\rtimes \text{CP}$, the models of ref.~\cite{Ding:2013hpa,Feruglio:2013hia} reproduce a nearly $\text{TM}_2$ mixing pattern while those of ref.~\cite{Li:2013jya}
come close to the $\text{TM}_1$ scheme. Other examples of models within $G=S_4\rtimes \text{CP}$ are those of ref.~\cite{Luhn:2013vna,Li:2014eia,Penedo:2017vtf,Ding:2018tuj}.
\subsubsection{$\Delta(3 n^2)$ and $\Delta(6 n^2)$}
The groups $A_4$ and $S_4$ are particular cases of the series $\Delta(3 n^2)$ and $\Delta(6 n^2)$, respectively, realized with the choice $n=2$.
General results for the whole series have been given in ref.~\cite{Hagedorn:2014wha,Ding:2014ora,Ding:2015rwa,deMedeirosVarzielas:2017ote,Joshipura:2018rit}. For $G=\Delta(3 n^2)\rtimes \text{CP}$ broken into
$G_e=Z_3$ and $G_\nu=Z_2\times \text{CP}$ the mixing pattern is still of $\text{TM}_2$ type and depends on a continuous parameter. When $G=\Delta(6 n^2)\rtimes \text{CP}$ breaks into 
$G_e=Z_3$ and $G_\nu=Z_2\times \text{CP}$, also more complex mixing patterns arise, beyond the trimaximal one. 
The particular cases $G=\Delta(48)\rtimes \text{CP}$ and $G=\Delta(96)\rtimes \text{CP}$ have also been comprehensively studied in ref.~\cite{Ding:2013nsa,Ding:2014hva} and \cite{Ding:2014ssa}, respectively. As an example of an interesting mixing pattern,
we show in table \ref{tabH} the predictions of a particular case arising in $G=\Delta(384)\rtimes \text{CP}$ when choosing $G_e=Z_3$ and $G_\nu=Z_2\times \text{CP}$. On top of one real continuous parameter $\theta$, they depend on two discrete parameters $m$ and $s$, specifying the embedding of the $Z_2$ and CP transformations, respectively, within 
$\Delta(384)$.
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
$s$&$\sin^2 \theta_{13}$&$\sin^2 \theta_{12}$&$\sin^2 \theta_{23}$&$\sin\delta$&$|\sin\alpha|=|\sin\beta|$\\
\hline
$s=1$&$0.0220$&$0.318$&$0.579$&$0.936$&$1/\sqrt{2}$\\
&$0.0220$&$0.318$&$0.421$&$-0.936$&$1/\sqrt{2}$\\
\hline
$s=2$&$0.0216$&$0.319$&$0.645$&$-0.739$&$1$\\
\hline
$s=4$&$0.0220$&$0.318$&$0.5$&$\mp 1$&$0$\\
\hline
\end{tabular}
\caption{Results for lepton mixing parameters from $G_f=\Delta (384)$, $m=4$ and different CP transformations $X(s)$
\cite{Hagedorn:2014wha}. 
The continuous parameter $\theta$ has been optimized to reproduce $\sin^2\theta_{13}$. }
\label{tabH}
\end{table}
Good agreement with the mixing angles is obtained if $|\sin\delta|$ is large and $m=4$.
In this case the bound $|\sin\delta|>0.71$ holds. This mixing pattern is of $\text{TM}_1$ type.
For $s = 1$ and $s=2$ the parameter $|m_{ee}|$ relevant for neutrinoless double beta decay has a non-trivial lower bound, whereas for $s=4$
both Majorana phases are trivial and a cancellation cannot be avoided for normal ordering of neutrino masses. Apart from the constraints on CP phases also the lepton mixing angles are strongly restricted, which further sharpen the prediction of $|m_{ee}|$. 
\subsubsection{Other examples}
A remnant CP symmetry in combination with texture zeros has been examined in ref.~\cite{Barreiros:2018bju}. In the case of $G=A_5\rtimes \text{CP}$, one-parameter families of PMNS matrices have been studied \cite{Li:2015jxa,DiIura:2015kfa,Ballett:2015wia,DiIura:2018fnk,Lopez-Ibanez:2019rgb}, typically having trivial or maximal Dirac CP phase and trivial
Majorana phases. This study has been generalized in ref.~\cite{Turner:2015uta} to include lepton mixing matrices depending on three parameters. 
Other groups that have been combined with CP invariance include $T'$ \cite{Girardi:2013sza}, $\Delta(27)$ \cite{Nishi:2013jqa}, the series $D^{(1)}_{9n, 3n}$ \cite{Li:2016ppt}, $\Sigma(36\times 3)$ \cite{Rong:2016cpk}, $\text{PSL}_2(7)$ \cite{Rong:2019ubh}. Variants of the above setup exploiting a generalized CP symmetry have been
considered in refs.~\cite{Girardi:2016zwz,Chen:2018lsv,Ding:2018fyz}.
In ref.~\cite{Yao:2016zev} a scan of all groups of order less than 2000 has been performed,
assuming either $(G_e,G_\nu)=(Z_{m_1}\times \ldots \times Z_{m_p},Z_2\times \text{CP})$ or 
$(G_e,G_\nu)=(Z_2\times \text{CP}',Z_2\times Z_2\times CP)$, with physical quantities depending on one continuous real parameter. The lepton mixing matrices in good agreement with data fall into eight different 
categories up to possible row and column permutations. These viable mixing patterns can be 
reproduced starting from the discrete flavour groups $\Delta(6n^2)$, $D^{(1)}_{9n, 3n}$, $A_5$ and $\text{PSL}_2(7)$ combined with $CP$ symmetry. Most of them are of $\text{TM}_2$ type or deformation thereof. Exceptions are those
related to the survival symmetries $(G_e,G_\nu)=(Z_2\times CP',Z_2\times Z_2\times \text{CP})$ or those derivable from $A_5\rtimes \text{CP}$. 

If we assume $G_e=Z_{m_1}\times \ldots \times Z_{m_p}$ and  $G_\nu=Z_2\times Z_2\times \text{CP}$
in the neutrino sector, we potentially end up with the most predictive scenario, as shown in the first row of table \ref{tableCP}.
In this case, after specifying the embedding of the residual groups $Z_{m_1}\times \ldots \times Z_{m_p}$ and $Z_2\times Z_2$ in the full flavour group $G$, the PMNS matrix is fully determined, up to permutations of rows and columns. However, as shown in ref.~\cite{King:2014rwa,Chen:2015nha}, in this case the only viable PMNS matrix can only be of trimaximal $\text{TM}_2$ type
with trivial $\delta$, $\alpha_{31}=0$ and $\alpha_{21}$ a rational multiple of $\pi$. 
The relations (\ref{eq:relTM2}) with $\tan\delta=0$ and the relative comments apply.
The inverse problem of determining the most general residual CP symmetry of the neutrino sector compatible
with the present data has been studied in ref.~\cite{Everett:2015oka,Everett:2016jsk} and, assuming tribimaximal mixing, in refs.~\cite{Chen:2018zbq,Chen:2019fgb}. 
For a generic PMNS matrix, it is however not guaranteed that the residual symmetries of the neutrino and charged lepton sectors fit into a finite group.



The possibility of exploiting invariance under CP to predict or constrain physical phases find a natural application in the
context of leptogenesis. This aspect has been analyzed in refs.~\cite{Chen:2016ptr,Hagedorn:2016lva,Li:2017zmk,Hagedorn:2017wjy,Samanta:2018efa}. Flavour symmetries embedding CP have been also applied to the more general problem of simultaneously describing quarks and lepton masses \cite{Li:2017abz,Lu:2018oxc,Hagedorn:2018gpw,Hagedorn:2018bzo,Lu:2019gqp}. Indeed, taking quarks into  account is unavoidable. Whereas the latter could in principle be invariant under the action of a standard flavour group operating on the lepton sector, a CP-symmetry must transform all fermion fields. Its spontaneous breaking in the quark sector must also be assured, in order to reproduce the observed CP-violation in the CKM matrix.


\subsection{Outlook}
The embedding of CP into the flavour symmetry provides a valuable complement to the setup dealing with
ordinary flavour groups, fully commuting with the proper Poincar\'e transformations. In such more restricted 
framework lepton mixing angles, Dirac and Majorana phases can all be predicted simultaneously, in terms of a single
continuous real parameter in the most realistic and predictive cases. Many explicit models support the viability of such
approach, with similar disadvantages affecting models dealing with ordinary flavour groups:
a complicated symmetry breaking sector, additional auxiliary symmetries and fields to trigger the desired
pattern of symmetry breaking and a limited accuracy of the predictions due to higher dimensional operators. 



==> intro_original.tex <==
The observation and study of neutrino oscillations have established that neutrinos are massive. Two independent squared
mass differences and three lepton mixing angles have been determined with an accuracy approaching the percent level, moving the whole field into a precision era. Most of the experimental results can be coherently
interpreted in the context of three light active neutrinos and CPT invariance. Experiments sensitive to solar, 
atmospheric, reactor and accelerator neutrinos provide a consistent picture supported by many redundant tests. 
In table \ref{tableData} we report the results of recent fits to the oscillation parameters. Notation and conventions are those of the PDG \cite{PhysRevD.98.030001}, unless otherwise stated. Most remarkably, the mixing pattern in the lepton sector appears to be 
totally different from that in the quark sector, with two large mixing angles and a third one similar in size to the Cabibbo angle.

Very interestingly, global analysis start to be sensitive both to the mass ordering and to the Dirac CP violating phase
$\delta$. A preference for the normal mass ordering (NO) over the inverted one (IO) is emerging \textcolor{red}{from the data}, at the level of about 3 $\sigma$.
The best fit value for the Dirac CP violating phase is $\delta \approx (1.2\div 1.3) \pi$ (for NO), but uncertainties are large and CP conservation is still allowed within $2\sigma$. 
\begin{table}[h!] 
\centering
\begin{tabular}{|c|c|c|}
\hline
&{\tt Normal Ordering}&{\tt Inverted Ordering}\rule[-2ex]{0pt}{5ex}\\
\hline
$\sin^2\theta_{12}$&$0.310^{+0.013}_{-0.012}$&$0.310^{+0.013}_{-0.012}$\rule[-2ex]{0pt}{5ex}\\
\hline
$\sin^2\theta_{23}$&$0.563^{+0.018}_{-0.024}$&$0.565^{+0.017}_{-0.022}$\rule[-2ex]{0pt}{5ex}\\
\hline
$\sin^2\theta_{13}$&$0.02237^{+0.00066}_{-0.00065}$&$0.02259^{+0.00065}_{-0.00065}$\rule[-2ex]{0pt}{5ex}\\
\hline 
$\delta/\pi$&$1.23^{+0.22}_{-0.16}$&$1.57^{+0.13}_{-0.14}$\rule[-2ex]{0pt}{5ex}\\
\hline
$\Delta m^2_{21}/10^{-5}$eV$^2$&$7.39^{+0.21}_{-0.20}$&$7.39^{+0.21}_{-0.20}$\rule[-2ex]{0pt}{5ex}\\
\hline
$\Delta m^2_{3\ell}/10^{-3}$eV$^2$&$2.528^{+0.029}_{-0.031}$&$-2.510^{+0.030}_{-0.031}$\rule[-2ex]{0pt}{5ex}\\
\hline
\end{tabular}
\caption{Best fit values and 1$\sigma$ errors of the three-flavour oscillation parameters in the global analysis of ref. \cite{Esteban:2018azc}. The results include data on atmospheric neutrinos provided by the Super-Kamiokande collaboration.  There is a difference of $\Delta\chi^2(\text{IO}-\text{NO})=10.4$ between 
inverted ordering (IO) and normal ordering (NO). Note that $\Delta m^2_{3\ell}=\Delta m^2_{31}>0$ for NO and $\Delta m^2_{3\ell}=\Delta m^2_{32}<0$ for IO. For other recent global analysis, see refs. \cite{Gariazzo:2018pei,deSalas:2018bym,Capozzi:2019vbz}.}
\label{tableData}
\end{table}

Dedicated experiments have been planned to determine the mass ordering and $\delta$.
Mass ordering measurements with an individual significance of more than 3$\sigma$ could be realized with several different technologies and methods, exploiting atmospheric (KM3NeT/ORCA, PINGU, INO), reactor (JUNO) and accelerator (DUNE, Hyper-K) neutrinos.
DUNE and Hyper-K have planned sensitivities to CP-violation higher than 5$\sigma$ for most of the allowed range, even though a precise determination of $\delta$ around the maximal value will be very challenging.

The absolute neutrino mass scale is still unknown, though well constrained by both laboratory  and cosmological  observations. The current \textcolor{magenta}{laboratory limit $m_\nu=\sqrt{\sum_i |U_{ei}|^2 m_i^2} < 1.1$ eV (90\% CL),} recently set by the KATRIN experiment \cite{Aker:2019uuj}, is expected to be further improved in the future. At present cosmology provides the most stringent bound on the sum of neutrino masses,
$\sum_i m_i<0.12\div 0.68$ eV, though subject to uncertainties inherent to the adopted cosmological model, the number of free parameters used to fit observations and the actual set of data included in the analysis \cite{PhysRevD.98.030001}. Upper bounds on neutrino masses become weaker when the data are analyzed in the context of extended cosmological models, or when a conservative set of data is used, but not considerably weaker. 
These bounds are expected to improve significantly over the next years, thanks to the new planned experiments.
If the $\Lambda$CDM model of the universe is confirmed, and if neutrinos have standard properties, non-vanishing neutrino masses should be detected at the level of at least 3$\sigma$ \cite{PhysRevD.98.030001}.

The impressive suppression of neutrino masses is quite peculiar, even compared to that of the lightest charged fermions. Not only the electron mass is suppressed by ``only'' a factor $\ord{10^{5}}$ but, more important, the latter suppression follows from the inter-family hierarchy displayed by charged fermion masses, with subsequent families \refc{separated by only} about two orders of magnitudes. Conversely, all the three neutrino families are separated from the electroweak scale by at least 11 orders of magnitude. \textcolor{magenta}{The striking size of neutrino masses might be related to the possibility that the total lepton number $L$ is violated, though this is certainly not the only possible explanation.}
The violation of the individual lepton numbers have been established, but we still do not know whether $L$ is violated or not in Nature. The experimental clarification of this central aspect might shed light on the possible origin of flavour. Indeed from the theory viewpoint the simplest explanation of the smallness of neutrino masses is in term of the violation of $L$ at a very large scale,
possibly not far from the grand unified scale. Experimentally, the most promising $L$-violating transition is the neutrinoless double beta ($0\nu\beta\beta$) decay.
If interpreted in the context of \textcolor{red}{three light Majorana neutrinos}, the present experiments allow to set an \textcolor{magenta}{upper bound on $|m_{ee}|=|\sum_i U_{ei}^2 m_i|$,}
a combination of neutrino masses, mixing angles and Majorana phases. Despite the uncertainties due to the lack of knowledge 
of absolute masses and Majorana phases, $|m_{ee}|$ can be constrained by neutrino oscillation data alone and, at least for the case
of IO, the allowed region is getting closer and closer to the range explored by the present $0\nu\beta\beta$ decay experiments.
In table \ref{nonenubb} we report some of the most recent experimental results. We refer the \textcolor{red}{interested reader} to the recent reviews \cite{Pas:2015eia,DellOro:2016tmg,Vergados:2016hso,Dolinski:2019nrj}.
\begin{table}[h!] 
\centering
\begin{tabular}{|c|c|c|c|}
\hline
{\tt Isotope}& {\tt Lower Bound on} $T_{1/2}^{0\nu}$ ($\rm{yr}$)&{\tt Upper Bound on} $|m_{ee}|$ ($\rm{meV}$)&{\tt Collaboration}\rule[-2ex]{0pt}{5ex}\\
\hline
$^{76}$Ge&$8.0\cdot 10^{25}$ &$120\div260$& GERDA\rule[-2ex]{0pt}{5ex}\\
\hline
$^{130}$Te& $1.5\cdot 10^{25}$&$110\div520$& CUORE\rule[-2ex]{0pt}{5ex}\\
\hline
$^{136}$Xe& $1.07\cdot 10^{26}$&$61\div165$& KAMLAND Zen\rule[-2ex]{0pt}{5ex}\\
\hline
$^{136}$Xe& $3.5\cdot 10^{25}$&$93\div286$& EXO 200\rule[-2ex]{0pt}{5ex}\\
\hline
\end{tabular}
\caption{Lower bound on $T_{1/2}^{0\nu}$ (90\% CL) and upper bound on $|m_{ee}|$ from GERDA \cite{Agostini:2018tnm}, CUORE \cite{Alduino:2017ehq}, KAMLAND Zen \cite{KamLAND-Zen:2016pfg}, EXO 200 \cite{Anton:2019wmi}. The quoted range reflects the uncertainty
in the nuclear matrix elements required to translate the half-life $T_{1/2}^{0\nu}$ into $|m_{ee}|$.}
\label{nonenubb}
\end{table}

Few experimental anomalies are still looking for more observational support or a coherent theoretical interpretation.
These include: i) the so-called reactor anomaly \cite{Mention:2011rk}, i.e.\ the evidence for disappearance of electron antineutrinos 
in short baseline experiments; ii) the Gallium anomaly \cite{Abdurashitov:1998ne,Abdurashitov:2005tb,Kaether:2010ag}, i.e.\ the observed deficit in the Gallium radioactive source experiments;
iii) the indications for $\nu_\mu\to \nu_e$ conversion from the LSND \cite{Aguilar:2001ty} and MiniBoone \cite{Aguilar-Arevalo:2018gpe} experiments. Taken at face value, these effects do not fit the standard
framework with three light neutrinos and explanations invoking a fourth sterile neutrino have been adopted. 
Even in such an extended scheme the anomalies do not find a coherent interpretation,
due to the tensions between appearance and disappearance data \cite{Dentler:2018sju}, indicating either
the need for a less minimal framework or the invalidation of some of the experiments.
While the discovery of a sterile neutrino would represent a major \textcolor{red}{result} of the current experimental activity
and a non-trivial challenge for its interpretation in the context of the flavour puzzle, here we will assume a low-energy framework
with three light active neutrinos and CPT invariance. New states are not excluded, but are assumed to be heavy,
allowing for an effective description of the current experiments where only the light degrees of freedom take action.

There are few theoretical tools allowing a quantitative and predictive description of neutrino mass and mixing parameters. Among them flavour symmetries are one of the most appealing option, given the role that symmetries have played in accounting for the properties of fundamental interactions. In this review we will
focus on flavour symmetries applied to the lepton sector. There are many good surveys of the subject \cite{Altarelli:2010gt,Ishimori:2010au,Smirnov:2011jv,King:2013eh,King:2014nza,King:2017guk,Petcov:2017ggy,Xing:2019vks}.
In the present work beyond incorporating the most recent developments of the field, we have provided a general classification of flavour symmetries, meant to cover not only the lepton sector but the whole fermion area. The latter feature, peculiar of this review, is particularly relevant to clearly identify the uncharted directions from the already explored ones. After recalling the possible origin of neutrino masses in section II, in section III we classify the possible flavour symmetries according to whether or not they commute with the Poincar\'e and gauge groups and according to their linear or nonlinear action in field space. In this section we also discuss general aspects of symmetry breaking, reporting elements of the theory of invariants where this problem finds 
its more natural mathematical formulation. The following sections, IV, V and VI provide a more specific
description and several illustrative examples of the type of symmetries classified in section III. Finally in section VII we summarize our personal thoughts on the subject. 

There are many related topics that we have only briefly mentioned or deliberately left out of this work. This list is long and includes radiatively generated neutrino masses, renormalization flow effects, extension to the quark sector also within grand unified theories or string theory, realization in the context of extra dimensions, relation to lepton flavour violation searches and leptogenesis, mathematical aspects such as group theory. We refer the reader to the mentioned literature.
 











